Serverless Data Science -- Are We There Yet? A Case Study of Model Serving

Machine learning (ML) is an important part of modern data science applications. Data scientists today have to manage the end-to-end ML life cycle that includes both model training and model serving, the latter of which is essential, as it makes their works available to end-users. Systems of model serving require high performance, low cost, and ease of management. Cloud providers are already offering model serving choices, including managed services and self-rented servers. Recently, serverless computing, whose advantages include high elasticity and a fine-grained cost model, brings another option for model serving. Our goal in this paper is to examine the viability of serverless as a mainstream model serving platform. To this end, we first conduct a comprehensive evaluation of the performance and cost of serverless against other model serving systems on Amazon Web Service and Google Cloud Platform. We find that serverless outperforms many cloud-based alternatives. Further, there are settings under which it even achieves better performance than GPU-based systems. Next, we present the design space of serverless model serving, which comprises multiple dimensions, including cloud platforms, serving runtimes, and other function-specific parameters. For each dimension, we analyze the impact of different choices and provide suggestions for data scientists to better utilize serverless model serving. Finally, we discuss challenges and opportunities in building a more practical serverless model serving system.

==> sections/related-work.tex <==
\section{Related Work}\label{sec:related-work}

\textcolor{blue}{(Need to update this section.)}
The most related work to ours is MArK~\cite{mark}, which mainly evaluates the cost of several model serving systems on the cloud. However, it does not investigate the performance of existing serverless systems and the data security in serverless model serving. 

%Mark~\cite{mark} is the most relevant study to our work. It evaluated the cost of machine learning model serving on the cloud with Function-as-a-Service(FaaS), Container-as-a-Service(CaaS) and Instance-as-a-Service(IaaS) offering. And It focused on the cost performance trade-off for different configuration of IaaS including, instance type, hardware accelerator and request batching. But they did not comprehensively evaluate these systems under fluctuating workload which is more realistic and meaningful for online prediction. Our work reveals the superior scalability of FaaS and its advantage in busrty model serving workload with a reasonable increase of cost. They built Mark which scales AWS EC2 instances with workload prediction and use AWS Lambda as backup to handle burst of request. Our insights also suggest the combination of FaaS and IaaS can reduces overall cost of model serving, but shows the potential of using primarily FaaS to handle request fluctuation under certain scenario.

\vspace{1mm}\noindent
\textbf{Service Level Objective (SLO).} 
There are a number of model serving systems focus on automatically select hardware configurations and models to improve accuracy or cost-effectiveness, under the constraint of SLO on latency. 
%FaaS with its unique cost performance profile, as shown in our study, introduces new design choices when building such model serving system on cloud.
Clipper~\cite{clipper} and Rafiki~\cite{rafiki} use an ensemble of models to navigate between accuracy and latency. They also adaptively batch prediction requests to boost throughput when the latency requirement is satisfied. 
%Clipper avoids high latency by caching and replying with fast models in the ensemble. Rafiki, when workload suddenly increases, reduces the number of models used for one request and use them to serve requests concurrently to reduce latency and failure rate. 
%
Swayam~\cite{swayam} presents an autoscaling framework that monitors the distribution of request execution time to proactively scale the number of CPU servers to meet the SLO requirement.
%
%%%comment out 20210223
%Yadwadkar, et al.~\cite{case-model-less} discussed the challenges of building a model serving system that navigate the complex design space of model variants, resource allocation among service, hardware characteristics and specifically highlighted hardware starting time being a important factor to cost efficiency. They built INFaaS~\cite{romero2019infaas} that generates models variants with different accuracy, resource consumption, and performance tradeoff and dynamically select model variant, scale up and down CPU/GPU servers, and share resources among different prediction services with respect to changing workload. 
%
BATCH~\cite{BATCH-serve} designs a mechanism that batches multiple requests and dynamically chooses the resource configuration of invoked serverless function, to satisfy latency constraint and minimize cost. None of these systems, however, address the data security problem for serverless model serving.

\begin{comment}%%%wyc: remove sgx part
\vspace{1mm}\noindent
\textbf{Secure serverless computing.}
There are several works focusing on security in serverless computing. 
%
S-FaaS~\cite{sfaas} uses SGX to enable trusted measurement of resource usages. S-FaaS proposes a Key Distributed Enclave (KDE) which performs similar functions to KEnclave in \name{}. However, KDE distributes the same keys to all users, therefore it is not secure under our threat model which considers malicious users. More importantly, S-FaaS suffers the same performance limitation as the naive design.  
%
\cite{systor19} utilizes a runtime inside the enclave to support multiple functions sharing the same enclave. However, it does not meet our deployability goal because it requires the cloud provider to handle key management between users and the enclave. Furthermore, it changes resource
management: current serverless systems use containers as the unit of resource management, whereas the unit is the sandboxes running inside enclaves in~\cite{systor19}. 
%
In addition, these works only consider simple functions inside enclave while our work focuses on the complex model serving scenario.

\vspace{1mm}\noindent
\textbf{Secure model serving.} There is another line of work~\cite{LeeLPLLLXXZS19,KimKR0CTL20} aiming at improving the efficiency for secure model serving inside the enclave, e.g., optimizing the enclave memory usage. 
%
Nevertheless, these works do not focus on the serverless computing paradigm, which brings new challenges in terms of performance and deployability. Besides, we note that these improvements to secure model serving could also be incorporated into our system as they are orthogonal to \name{}.
\end{comment}
% ~\cite{lambda-with-mlperf} modified MLPerf to evaluate feasibility of model inference on AWS lambda. They showed that latency drops as allocated function memory increases but this does not lead to increase in throughput. But they did not benchmark serverless function with other model serving options on the cloud or discuss the cost perspective.
